On the density regime probed by HCN emission

HCN J$\, =\,$1$\, -\,$0 emission is commonly used as a dense gas tracer, thought to mainly arise from gas with densities $\mathrm{\sim 10^4\ -\ 10^5\ cm^{-3}}$. This has made it a popular tracer in star formation studies. However, there is increasing evidence from observational surveys of `resolved' molecular clouds that HCN can trace more diffuse gas. We investigate the relationship between gas density and HCN emission through post-processing of high resolution magnetohydrodynamical simulations of cloud-cloud collisions. We find that HCN emission traces gas with a mean volumetric density of $\mathrm{\sim 3 \times 10^3\ cm^{-3}}$ and a median visual extinction of $\mathrm{\sim 5\ mag}$. We therefore predict a characteristic density that is an order of magnitude less than the "standard" characteristic density of $\mathrm{n \sim 3 \times 10^4\ cm^{-3}}$. Indeed, we find in some cases that there is clear HCN emission from the cloud even though there is no gas denser than this standard critical density. We derive luminosity-to-mass conversion factors for the amount of gas at $A_{\rm V} > 8$ or at densities $n > 2.85 \times 10^{3} \: {\rm cm^{-3}}$ or $n > 3 \times 10^{4} \: {\rm cm^{-3}}$, finding values of $\alpha_{\rm HCN} = 6.79, 8.62$ and $27.98 \: {\rm M_{\odot}} ({\rm K \, km \, s^{-1} \, pc^{2}})$, respectively. In some cases, the luminosity to mass conversion factor predicted mass in regions where in actuality there contains no mass.

==> ResponsetoReviewer.tex <==

I'd like to thank the Reviewer and the Assistant editor for the useful comments on this paper. We also appreciate the swift response to the review of this paper. Whilst we agree on several points the reviewer has raised (and therefore addressed) we do disagree with a few comments and we therefore put forward our rebuttal to those comments below here. All the amendments to the paper have highlighted in bold in the new version of the manuscript.

** The HCN/CO ratio in Eq.(3)

  The HCN/CO ratio is fundamental to the present work since the HCN
  abundance is derived from that of CO based on this ratio. It is
  assumed that the ratio is driven by the visual extinction, Av (see
  Fig. 1 and Eq. 3). The value of this ratio as a function of Av,
  $\Phi{(Av)}$ in Eq.3, is obtained from Fuente et al 2019. However, in
  this paper, the HCN/CO ratio is investigated in terms of three
  control parameters: Av, cosmic-ray ionization rate (zeta), C/O, and
  sulfur abundance (S/H). This is Fig. 8 of that paper. As is clearer
  apparent, the ratio primarily depends on the C/O and S/H ratios,
  not on Av, nor on zeta. Therefore, based on Fuente et al 2019, one
  should take $\Phi(Av)$ = constant; the value of the constant being
  determined by the carbon budget (C/H). I do not expect the main
  results of this work to be drastically changed, but it is clear
  that Eq.(3) of the paper is not justified.

  The models should be redone with $\Phi{(Av)}$ = constant for a given C/O.

Perhaps the reviewer has misunderstood what we are doing with our HCN abundances. We are using the  *observed* correlation between  x(HCN)/x(CO) and Av — the same points that are displayed in the figure you refer to: Fig 8 of Fuente et al. 2019.  While it's true that the modelling does not demonstrate a correlation between x(HCN)/x(CO) and Av, the observed data clearly does. Yes, this could be explained variations in the abundance of C from region to region, as shown in the models — the left-most panels in Fuente's Fig 8 —  but it could also quite easily be explained by other factors not explored in their modelling, such as variations in density, the complicated relation between density and Av, and the time history of the chemistry (clouds aren't static, as typically assumed in chemical modelling).

All things considered, we felt that it was more appropriate here to take the observations at face value, connecting the abundance of HCN to x(CO), which is followed self-consistently in the code (and actually with a C/H consistent with model A in Fuente), and to the line-of-sight Av in the RT set-up.  Even so, it's worth stressing here that this approach is conservative. The slight Av dependency that we introduce actually enhances the HCN abundance at high Av and decreases it low Av. If we were to remove it, our results would show HCN tracing even lower densities. We have now made it clear in the text that we are fitting to the observed data from Fuente et al. 

Given the high computational cost of re-running these models — each takes ~48+ hours to run, and there are 120 of them! — we would prefer to keep things as they are. We believe what we have done is consistent with the available observational data, and the reviewer's suggestion, while valid, is unlikely to alter the main conclusions of the paper. We'd also note to the reviewer than we are currently working on using a much more sophisticated treatment of the chemistry -- using tracer particles from Arepo as input to the UCLChem code. Unfortunately this has thrown up some challenges and so is taking longer than we'd like, but the preliminary results suggest that the HCN abundances used in our current study are fairly robust. 


  I do not understand the statement p5 l57 "demonstrating that our
  HCN abundance treatment is appropriate for this study." This is an
  internal consistency check, not a proof that the HCN abundance is
  correct.

We have removed this sentence as it was, as the reviewer points out, confusing. 


*In response to the C/O ratio
  Since this is the main driver of the HCN/CO ratio -- this is indeed
  stated in the Fuente et al 2019 paper, in the last paragraph on
  page 10 -- and since this is a free parameter in the present
  simulations, it would be more interesting to investigate the effect
  of this ratio on the HCN emissivity. The present models were done
  with C/O=0.44, which is fine. However, it is well known that C/O up
  to 1 can not be ruled out (see, for instance, Fuente et al).

We agree that a study looking at the variations in the metallicity would be informative, especially as the C/O ratio can vary quite a bit. However we feel that this is significantly outside the scope of this study. In fact, it would constitute an entirely separate study to the one we do here. First, we would need to re-run all of the MHD simulations for each variation in the abundances, as the cooling in the gas depends on the abundance of both C and O, via  emission from [CII], [CI] and CO (and via [OI] in a galactic centre/starburst environment -- Clark et al. 2013 --  or at very low metallicity -- Glover & Clark 2012). Then, we would need to re-run all the RT simulations for each metallicity. This on its own would constitute a larger paper than the one we present here. Given that HCN emission is likely to be more sensitive to the gas temperature (set by G0 and the cosmic ray ionisation rate), it's also not clear that such a study would be a priority. We are planning on looking at this however, and have already started investigating the HCN emission with varying G0/CRs. 

** Nature of the gas traced by HCN
 The main goal of the paper is to determine the density regime
  traced by HCN with the background question to relate the HCN
  luminosity to the star forming efficiency. This thus requires to
  know the mass traced by HCN compared to the total mass of gas. As
  stated in the Introduction, it is not clear what "gas available for
  star formation" means.

  But I am not sure the way this is investigated really addresses the
  question. I know this is a common way to do so (e.g. Krumholz and
  Thompson 2007). Yet, the integrated intensity is not only a
  function of density, and the emergent integrated intensity, W$\_{tot}$,
  is not simply the sum of the W$_i$ of each cell; in other words,
  zeroing the cells with n>n$_{thr}$ and compute the emergent spectrum
  does not give, in general, the same result as zeroing the cells
  with n   are interested in the latter procedure, namely suppress the
  contribution of cells with n   both procedures should give the same, that is the cumulative
  fraction will be one minus that shown in Fig. 7. But in general, I
  do not expect this to be true.

  In the present state, the paper does not clarify these aspects
  which are, however, crucial to both the understanding of the
  method, and the impact of the results.

  I would like to see the equivalent of Fig. 7 but done the other way
  around, as suggested above.

  I would also like to see a plot of I(z) and W(z), with z the
  coordinate along a given line of sight. I expect to this to show
  the contribution to the emergent HCN luminosity of the various
  regions along the los. This could obviously be repeated for a bunch
  of los, and then make some statistics from it. I guess the authors
  have already tried this in which case I would be interesting in
  knowing why this was not retained.

Unfortunately the reviewer's comment here is a little unclear — we think they are saying that we should be removing HCN *below* a certain density in our analysis, rather than *above*, as we claimed in the text. This is actually indeed what we have done, and we apologise for the confusion: there was a typo in our original manuscript, which has now been fixed.  Clearly carving out holes in the cloud's HCN abundance at high densities would not be representative of reality: yes, the abundance can drop at high densities due to depletion, but this is only expected to occur at the very highest densities we probe in our RT analysis. Carving out "voids" of HCN in high density gas is thus an unphysical representation of a cloud, whereas removing the lower density HCN provides a more physically probable model of a molecular cloud. 

We also do understand that removing the emission from the low density regions will alter the amount of emission in a non-uniform way. However for RADMC-3D, which uses the LVG method for working out the level populations, this shouldn't be a large effect: with LVG the level populations are worked out *first*, depending only on *local* properties of the radiation field — i.e. there is no self consistent (and iterative) coupling of the population levels to the incoming radiation field. We hope this is clear to the reviewer.

The other plots that the reviewer is requesting — i.e. I(z) and W(z) along the line of sight —  aren't possible with RADMC-3D, unfortunately.  We do however agree that they would be informative. How exactly one makes a plot of I(z) isn't clear though, even if the information was available: we need to do this for each of the 400-off velocity channels, for each line of sight! 

Regarding the opening section of the reviewer's comment, we stress that there are *numerous* studies, many extremely impactful, that use HCN as a tracer — and indeed measure of the mass contained in —  "high density gas". These studies explore correlations between the star formation rate and the mass in this dense gas. What is not clear from these studies is what density HCN actually traces  — i.e. what "high density" actually means —  or indeed whether breaching such a density means that 'gas is available for star formation'. The purpose of the paper is to ask what density (and column density) regime the HCN probes; given that most observations of HCN are 'unresolved' (i.e. the regions emitting are not filling the beam and contain substantial variations in density, temperature, and emissivity of HCN), we think this is an important study. We do not examine whether this constitutes 'the gas available for star formation' in this study, as this is a separate, and actually quite difficult thing to disentangle from the simulations -- and one that has still to be done!


** HCN distribution in the clouds and emergent spectra

  This comment is related to the previous point. I find it
  frustrating that the paper does not provide clues about the
  distribution of HCN (abundance), the opacity of the HCN line,
  spectral line shape; the column density of HCN is also never shown
  or given quantitatively. Yet this determines the opacity of the HCN
  lines. For instance: what is the column density of the low-density
  regions that sum up to ~50% of the total integrated emission?

First, regarding the column densities of the HCN emission, we have an entire section devoted to this and Figures 9 and 10 give exactly the information that the reviewer requests.  Please check that this suffices. 

We debated including information on the HCN abundances, but given that they are prescriptive, we originally decided to leave them out. We have now included a figure  (Figure 5) showing the column density of the HCN. 

We also agree that a line profile would be helpful for observers, to aid comparison with their studies; we include line profiles from each of our clouds in Figure 13. 



" - It seems that many physical quantities that should be in math mode
   are not;"
   
We try to be as consistent as possible with the use of math mode however this might be something that the editor could possibly smooth out as we do not see these problems.
   
" - The last sentence of the abstract should be rephrased;"

We have decided to remove the last sentence of the abstract as it was restating a point that was made earlier in the abstract.

"- p2 l40: the second 10$^3$ should probably be 10$^4$ cm-3"

The second 10$^3$ should be 10$^3$ as it is two different papers that conclude the same density of ~10$^3$.

"- p3 l44: please give the corresponding C/O"

The elemental abundances of both carbon and oxygen were given in the second last paragraph of Section 2.2. 

"- p3 l47 right column (RC): "can the be used" -> "then be used" ?"

Amended in paper

" - p3 l62 RC: in practise -> in practice
  - Stop here for the typos. Please perform thorough proof-reading."

Many thanks. We've looked through the paper many times and have tried to pick up as many typos as we can.  

" - p4 l27 RC: I do not understand what "the dense gas [...] is
   actively destroyed"; what do you mean?"

This is a common feature of turbulence in that small density fluctuations are ripped apart by ram-pressure from the very flows that initially created them. We have re-worded this section. 

" - p4 l38 RC: "have therefore evolved far enough to proceed...": the
   chemical timescales of HCN and CO are not necessarily identical,
   and indeed, one expects that of HCN to be slightly longer; in any
   instance, a comment is needed to discuss the dynamical and the
   chemical timescale of CO (which drives that of HCN in these
   calculations);"

Agreed. Priestley and Whitworth 2021 has looked at this, and found that the HCN forms quickly in the cloud collision. We have a) noted the caveat to our set-up and b) referred to their paper, which suggests the formation timescale is unlikely to be an issue with our study. 

" - Give the exact reference for the collision rate coefficients."

Exact reference now given.

" - Figures 7 and 8 are the same; they should be merged."

Figures 7 and 8 have been merged

" - Figure 8: caption; remove 'light green'; n$_{char}$ = 2.9E3 not E-3
   cm-3."

Corrected

" - I did not see where Fig. 9 was refereed to; probably unnecessary
   and could be removed. But if the Figure was kept, the line styles
   should be put on it explicitly."
   
We mistakenly did not reference the Figure and have now amended the paper. We believe it is quite a useful figure as it shows the fraction of high density (and column) of the gas in the radmc simulations very clearly in a cumulative (had it been a conventional cumulative the high density section would've been very difficult to read)

" - Figure 12 could be moved to an Appendix."

We feel that this Figure is an important part of the discussion of the numerical technique associated with the results in Section 4.2, and as such, we'd prefer to keep it in the main body of the paper, rather than have the reader search through the appendix for the information.

" - p10 l16 RC: remove "Once again, we assume...""

Removed

" - p10 l46 RC: "this combination is a much more..."; unclear"

Attempted to clarify in paper. But essentially we are trying to convey that using 5.05 mag is the best option compared to 8 mag.


" - p 10 last paragraph of Section 4.1: I did not find the previous
   calculations leading to Av=10 mag. On the other hand, Fig.10 gives
   5.05 mag for the characteristic Av of L$_{HCN}$."

Apologies, the reviewer is correct. We have fixed this in the text.


" - p11 l45 LC: I did not find where n$_{eff}$ was defined; please check."

Referenced Shirley as it gives a very good definition of neff.

" - p11 l60 LC: I could not find how is the ortho/para ratio of H2
   taken into account;"
   
Apologies — we neglected to quote our assumed ortho/para ratios. We have included the following sentence. "When calculating the level populations of the CO, we assume the gas has ratio of ortho to para H$_2$ ratio of 3:1 ". 
   
" - p13 l10: what does the HCN-to-HNC ratio bring to the discussion?"

We do not know what the reviewer is asking here. We were trying to point out that our HCN abundances are possibly lower than the Hacar et al. study would suggest, and that this might push the density traced by HCN to even lower values than we report in our study.

" - p13 l17: I thought there was a temperature-dependent abundance for
   CO and thus for HCN. Please clarify. "
 
We are unsure what the reviewer means here. The CO abundance, as stated in the numerics section, is  followed self-consistently in the code and we tie the HCN abundance to the CO abundance via Equation 3. While there will undoubtedly be a correlation between CO abundance and temperature in our models (e.g. see figures 2 & 3 together in Clark et al. 2019), we do not enforce one in any way in this study.  


" - p13 l31 LC: that Fuente+19 gives a "very conservative estimate for
   the HCN abundance" remains to be proved; again, these authors show
   that HCN/CO depends on the C/O more than on Av. :
   
We believe that this has been answered previously and that the statement in the paper holds.
   
   
Both errors below have been amended :-
   
 - p13 l48 LC: "3 x 10$^4$ cm-3"; did you mean :2.85E3 cm-3?
 
 - Fig.15: W$_{CO}$ -> W$_{CO(1-0)}$; also, in the caption, line ratio ->
   integrated intensity ratio. 





